Optimal Robust Linear Regression in Nearly Linear Time

We study the problem of high-dimensional robust linear regression where a learner is given access to $n$ samples from the generative model $Y = \langle X,w^* \rangle + \epsilon$ (with $X \in \mathbb{R}^d$ and $\epsilon$ independent), in which an $\eta$ fraction of the samples have been adversarially corrupted. We propose estimators for this problem under two settings: (i) $X$ is L4-L2 hypercontractive, $\mathbb{E} [XX^\top]$ has bounded condition number and $\epsilon$ has bounded variance and (ii) $X$ is sub-Gaussian with identity second moment and $\epsilon$ is sub-Gaussian. In both settings, our estimators: (a) Achieve optimal sample complexities and recovery guarantees up to log factors and (b) Run in near linear time ($\tilde{O}(nd / \eta^6)$). Prior to our work, polynomial time algorithms achieving near optimal sample complexities were only known in the setting where $X$ is Gaussian with identity covariance and $\epsilon$ is Gaussian, and no linear time estimators were known for robust linear regression in any setting. Our estimators and their analysis leverage recent developments in the construction of faster algorithms for robust mean estimation to improve runtimes, and refined concentration of measure arguments alongside Gaussian rounding techniques to improve statistical sample complexities.

==> content/outline.tex <==
\section{Outline}
\Ninote{This section has to be cut-down to the essential}
\subsection{Algorithm Outline}

The rough meta-algorithm will proceed as follows:

\begin{algorithm}[H]
\caption{Linear Regression}
\label{alg:linreg}
\begin{algorithmic}[1]
\State \textbf{Input: } Set of sample points $Z_i =  (X_i, Y_i)$, Outlier Fraction $\eta$, Length of Parameter Vector $\norm{\beta}$
\State $nit \gets \nit$
\State $l \gets \tO(\frac{d \log \beta}{\eta^2})$
\State $\bm{Z} = \{(X_1, Y_1), \dots, (X_l, Y_l)\}$
\State Truncate samples which satisfy $\norm{X_i} \geq O(\sqrt{d})$
\State $w_0 \gets 0$
\For {$t = 0:nit$}
    \State $g_t \gets \gest (\bm{Z}, w_t)$
    \State $w_{t + 1} \gets w_t - \gamma g_t$
\EndFor
\State \textbf{Return: }$\Sigma^*$
\end{algorithmic}
\end{algorithm}

For the case where the samples are drawn from the distribution $Y = \inp{X}{\beta} + \epsilon$ where $X$ satisfies $L4-L2$ hypercontractivity with covariance matrix $\Sigma$ and $\eta$ is zero mean with variance $\sigma^2$, the gradient estimation steps can simply be calling the mean estimation algorithm on gradients; that is, we call a robust mean estimation algorithm on $G_i = (\inp{X_i}{w_t} - Y_i)X_i$. We see that under no adversarial corruption, $G_i$ is a random vector whose covariance matrix, $\Sigma_t$, has small spectral norm. For any $v$, we have:
\begin{align*}
    v^\top\Sigma_t v &\leq \mb{E} [(\inp{X_i}{w_t} - Y_i)^2 \inp{X_i}{v}^2] = \mb{E} [(\inp{X_i}{w_t - \beta} - \epsilon_i)^2 \inp{X_i}{v}^2] \\
    &= \mb{E} [(\inp{X_i}{w_t - \beta}^2 + \epsilon_i^2) \inp{X_i}{v}^2] \leq \norm{\Sigma} \sigma^2 + L \cdot \norm{\Sigma}^2 \norm{w_t - \beta}^2.
\end{align*}

Therefore, the robust mean estimation algorithm returns an estimate of the gradient upto an error of $O(\eta \norm{\Sigma} \sqrt{\sigma^2 + \norm{w_t - \beta}^2})$. Note that the true gradient is $\Sigma (w_t - \beta)$, which means that when the norm of the true gradient is significantly larger than the error rate, we obtain a good estimate of the gradient allowing us to improve our estimate. 

For subgaussian case (Both $X$ and $\epsilon$ are subgaussian) with identity covariance, the previous algorithm brings us to within $O(\sigma \sqrt{\eta})$ of the true parameter vector $\beta$. At this point, we have for any unit vector $v$:
\begin{equation*}
    v^\top \Sigma_t v \leq \mb{E} [(\inp{X_i}{w_t - \beta} - \epsilon_i)^2\inp{X_i}{v}^2] = \mb{E} [(\inp{X_i}{w_t - \beta}^2 + \epsilon_i^2)\inp{X_i}{v}^2] = \sigma^2 (1 + \tO(\epsilon)). 
\end{equation*}
Furthermore, note that each $G_i = (\inp{X_i}{w_t} - Y_i)X_i$ is sub-exponential. Therefore, we should be able to show that for any $(1 - O(\eta))n$ sized set of data points, the spectral norm of the covariance matrix formed by taking those samples is approximately $1 \pm \tO(\eta)$. Therefore, we should be able to improve our estimate to $\tO(\eta)$ by computing the following SDP:
\begin{equation*}
    \min_{s_i \in \mc{S}} \max_{M \succcurlyeq 0, Tr(M) = 1} \inp{M}{\sum s_i G_i G_i^\top}
\end{equation*}
where $\mc{S} = \{s_i: s_i \geq 0, \sum s_i = 1, s_i \leq 1 / ((1 - 10\eta)n)\}$. This should result in a value less than $1 + \tO(\eta)$ which is all you need for the mean $\sum s_i G_i$ to be an estimate of $w_t - \beta$ up to an error of $\tO (\sigma \eta)$ (the analogue from the termination of algorithm 1 and Lemma 3.2 from \href{https://arxiv.org/pdf/1811.09380.pdf}{here}). Interestingly, this phase of the algorithm is completed in 1 step without the need for doing the more intricate analysis from the paper. This also simplifies their mean estimation result for the sub-gaussian case.

To avoid reusing samples, we'd need a bound on the following quantity:

\begin{equation*}
    \max_{\norm{u} = 1} \min_{s_i} \max_{\norm{v} = 1} \sum_{i = 1}^k s_i \inp{M_i - \Sigma}{u \otimes v}^2 \leq c.
\end{equation*}


\subsection{Heavy Tailed Proof}
We have $\eta$ denoting the fraction of corruptions and $\epsilon$ denoting the noise in each sample. Furthermore, we will assume that the samples arise from a corrupted version of the distribution $Y = \inp{X}{w^*} + \epsilon$. where $X$ is zero mean and satisfies L2-L4 hypercontractivity with hypercontractivity constant $O(1)$ and has covariance matrix $\Sigma$ with $O(1)$ condition number. Formally, we will have the following assumptions:

\begin{assumption}
\label{as:htassumptemp}
We make the following assumptions on the data generating process:
\begin{enumerate}
    \item $X$ is a vector with covariance matrix $\Sigma$. Forthermore, $X$ is L4--L2 hyper contractive. That is, for all $\norm{u} = 1$, we have:
\begin{equation*}
    \mb{E} [\inp{u}{X}^4] \leq C_1 \cdot \lprp{\mb{E} [\inp{X}{u}^2]}^2
\end{equation*}
for an absolute constant $C_1$. For normalization purposes, we will assume $\norm{\Sigma} = 1$. 
    
    \item The condition number of $\Sigma$ is bounded by another absolute constant $C_2$. 
    
    \item The noise variable $\epsilon$ is zero mean and independent of $X$ with variance bounded by $\sigma^2$. 
\end{enumerate}
\end{assumption}

Suppose we have data points $(X_i, Y_i)_{i = 1}^n$ with $n = \tO (d / \eta^2)$. At any iterate $w_t$, our goal will be to obtain an estimate of the gradient at $w_t$ from the data points. Therefore, at $w_t$, we have gradient estimates $g_i = (\inp{X_i}{w_t} - Y_i)X_i = (\inp{X_i}{w_t - w^*} - \epsilon_i)X_i$. We will aim to do this by running Ilias' algorithm on the $g_i$. We know that Ilias' algorithm gives us a good estimate of the gradient assuming there exists a set of weights $0 \leq s_i \leq (1 + O(\eta)) / n$ satisfying:

\begin{equation*}
    \sum_{i = 1}^n s_i g_i \approx \Sigma (w_t - w^*),\ \sum_{i = 1}^n s_i g_i g_i^\top \leq O(1 + \norm{w_t - w^*}^2).
\end{equation*}

This is equal to the following condition: for every unit vector $u$, there exist a set of weights $s_i$ satisfying:

\begin{equation}
    \label{eq:scons}
    \norm{\sum_{i = 1}^n s_i X_i X_i^\top - \Sigma} \leq O(\sqrt{\eta}),\ \sum_{i = 1}^n s_i \inp{X_i}{u}^2 X_i X_i^\top \leq O(1).
\end{equation}

The usual way to do this is to assume that one is working with purely clean samples from the underlying distribution with no corruption. However, this will not work here to give us the right sample complexity. Take $u$ along one of the $X_i$ of length $\sqrt{d}$ and we see that the matrix $\norm{X_i}^2 X_iX_i^\top$ has spectral norm approximately $d^2$, therefore we'd need at least $d^2$ samples for this strategy to work. 

For the first result, we will try to establish the following lemma:

\begin{lemma}
    \label{lem:c1conctemp}
    Let $\{X_i\}_{i = 1}^n$ be truncated at level $O(\sqrt{\Tr \Sigma})$ which be drawn from the original uncorrupted distribution (which satisfies $L4-L2$) with $n = \tO (d / \eta^2)$. Then, with probability at least $1 - 1 / d^2$ for any set of $(1 - 10\eta) n$ samples, $S$, we have:
    \begin{equation*}
        (1 - O(\sqrt{\eta})) \Sigma \preccurlyeq \abs{S}^{-1} \sum_{i \in S} X_iX_i^\top \preccurlyeq (1 + O(\eta)) \Sigma. 
    \end{equation*}
\end{lemma}

\begin{proof}
The upper bound follows simply because $\sum_{i \in S} X_i X_i^\top \preccurlyeq \sum_{i=1}^{n} X_i X_i^\top$ and applying matrix Bernstein. 

For the lower bound, consider a grid of resolution $O(poly(\epsilon / d))$, $G$. And consider for $u \in G$, the random variable $Z = \inp{X}{u}^2$. We know from L4-L2 that variance of $Z$ is $O(1)$. Now, consider the $1 - 10 \eta$ percentile of the random variable $Z$, $q$. We see that with high probability from Hoeffding's inequality, at most $(1 - 5\eta)$ points will be in the range $[0, q]$. Now, also note again from L4-L2 that $q \leq O(1 / \sqrt{\eta})$ and that $\mb{E} [Z_i \bm{1} \lbrb{Z_i \leq q}] \geq \mb{E} [Z_i] - O(\sqrt{\eta})$ (From Cauchy Schwarz). Therefore, with high probability $((1 - O(\eta))n)^{-1} \sum_{i = 1}^n Z_i \bm{1} \lbrb{Z_i \leq q} \geq (1 - O(\sqrt{\eta}))$. Therefore, the lower bound follows as these are the smallest $(1 - 5\eta)n$ of the $Z_i$ and we pick some set of $(1 - \eta)n$ of the $Z_i$. By a union bound, this holds on the entire grid and finally, for a non-grid element, we use the closest grid element as a proxy and subtract the error incurred (The closest grid element is really close say $O((\epsilon / d)^{10})$ or something).


\end{proof}

The previous argument states that any set of $(1 - \eta)n$ points suffice to ensure the first condition. For the second condition, we want to show the following quantity is small:

\begin{equation*}
    \max_{\tr{M} = 1} \min_{0 \leq s_i \leq (1 + O(\eta)) / n} \inp*{\sum s_i \inp{X_i}{u}^2 X_i X_i^\top}{M} = \min_{0 \leq s_i \leq (1 + O(\eta)) / n} \max_{\tr{M} = 1} \inp*{\sum s_i \inp{X_i}{u}^2 X_i X_i^\top}{M}.
\end{equation*}

We will work with the first characterization and additionally assume that $M$ is a rank one matrix $vv^\top$ and show the following lemma:

\Ynote{I'll take the following two lemmas}
\begin{lemma}
    \label{lem:r1conctemp}
    When $n = \tO(d / \eta^2)$, we have with high probability that for all $\norm{u} = \norm{v} = 1$:
    \begin{equation*}
        n^{-1} \sum_{i = 1}^n Z_i \bm{1} \lbrb{Z_i \leq q} \leq O(1)
    \end{equation*}
    where $Z_i = \inp{X_i}{u}^2 \inp{X_i}{v}^2$, $q$ is $O(1 / \eta^2)$ and at least $(1 - \eta / 100)n$ elements are in the above sum. Furthermore, all the elements satisfy $\inp{X_i}{u} \leq O(1 / \sqrt{\eta})$ and $\inp{X_i}{v} \leq O(1 / \sqrt{\eta})$.
\end{lemma}

\begin{proof}
We again start by gridding over the $u$ and $v$ using a grid of resolution $O(poly(\epsilon / d))$. Now pick a particular $u, v$ in the grid and let $q^\prime = O(1 / \eta^2)$. We have with probability at least $\eta / 1000$ that $Z_i \in [0, q^\prime]$. Now, noting that the variance of $Z$ is $O(1 / \epsilon)$ \Enote{Are we sure about this? This looks like a 4th moment that might need an L8-L2 kind of contraction; like if we had $u=v$? Also, why would the variance of this thing depend on $\epsilon$ at all? Are you trying to make sure they are not aligned?} \Ynote{Oh. It's roughly an argument like this: $\mb{E} [\inp{X_i}{u}^2\inp{X_i}{v}^2] \leq O(1 / \epsilon) \mb{E} [\inp{X_i}{v}^2]$ as the $X_i$ are truncated based on $\inp{X_i}{u}$}, we get the result by Bernstein's bound for the particular $u$ and $v$. By an union bound the result follows over the whole grid and finally, the result for non-grid points, holds by choosing a close proxy in the grid for each non-grid point.
\end{proof}

The one remaining portion of the proof is to go from the above lemma to verifying the second condition of Equation~\ref{eq:scons}. The proof will go through a rounding argument applied to the matrix $M$. We will now prove the following lemma:

\begin{lemma}
    \label{lem:c2conctemp}
    When $n = \tO(d / \eta^2)$, we have with high probability that for all $\norm{u} = 1$ and psd $M$ with $\tr{M} = 1$:
    \begin{equation*}
        n^{-1} \sum Z_i \bm{1} \lbrb{Z_i \leq q} \leq O(1)
    \end{equation*}
    where $Z_i = \inp{X_i}{u}^2 \inp{X_iX_i^\top}{M}$, $q$ is $O(1 / \eta^2)$ and at least $(1 - \eta / 10)n$ elements are in the sum and $\inp{X_iX_i^\top}{M} \leq O(1 / \eta)$. 
\end{lemma}

\begin{proof}
    We will condition on the event in Lemma~\ref{lem:r1conc}. Now, let $\norm{u} = 1$ and let $M$ be trace-1 psd matrix. Let $g$ be a gaussian with covariance matrix $M$. Now, for any $i$, $Y_i = \inp{gg^\top}{X_iX_i^\top}$ is a $\chi^2$ random variable. We will first condition on $\norm{g} \leq 5$ (This happens with probability at least $90\%$). Also, the $\bm{P} (\inp{g}{X_i}^2 \geq 0.1 \inp{M}{X_iX_i^\top}) \geq 0.6$. Therefore, we finally have:
    \begin{equation*}
        \bm{P} (\inp{g}{X_i}^2 \geq 0.1 \inp{M}{X_iX_i^\top} \cap \norm{g} \leq 5) \geq 0.5.
    \end{equation*}
    From the above we can conclude by contradiction that the number of $i$ such $\inp{X_iX_i^\top}{M} \geq O(1 / \eta)$ is $\eta / 50$. Finally, to show that the sum is small, we have for $\inp{X_iX_i^\top}{M} \leq O(1 / \eta)$:
    \begin{equation*}
        \mb{E} [\inp{X_iX_i^\top}{u}^2\inp{X_iX_i^\top}{gg^\top} \bm{1} \lbrb{\inp{X_i}{g} \leq O(1 / \sqrt{\eta})}] \geq 0.5 \inp{X_i}{u}^2 \inp{M}{X_iX_i^\top}.
    \end{equation*}
    By summing over $i$ satisfying $\abs{\inp{X_i}{u}} \leq O(1 / \sqrt{\eta})$ in the previous equation, we derive an upper bound on the required quantity, proving the lemma.
    
\end{proof}

\subsection{Sub-Gaussian Robust Linear Regression}

\Ynote{Efe, could you take the lemmas in this section?}
Similar to the previous setup, we will make the following stronger assumptions on the data generating process:

\begin{assumption}
\label{as:sgassump}
We make the following assumptions on the data generating process:
\begin{enumerate}
    \item $X$ is a zero mean random vector with covariance matrix $I$. Furthermore, we assume that $X$ is sub-gaussian with sub-gaussianity parameter bounded by $O(1)$. 
    
    \item The noise variable $\epsilon$ is zero mean, independent of $X$ and sub-gaussian with sub-gaussianity parameter bounded by $\sigma$. 
\end{enumerate}
\end{assumption}

Note that from the previous part, we can assume that we have an estimate, $w$ within $O(\sqrt{\eta} \sigma)$ of $w^*$. Therefore, we may now assume that $\norm{w^*} \leq O(\sqrt{\eta}\sigma$. As before, we will have to show that there exist a set of weights $0 \leq s_i \leq (1 + O(\epsilon)) / n$ satisfying:

\Ynote{Fill in appropriate logarithmic dependencies later.}
\begin{equation}
    \norm*{\sum_{i = 1}^n s_i Y_i X_i - w^*} \leq \sigma \tO (\eta),\ \norm*{\sum_{i = 1}^n s_i (Y_i X_i) (Y_i X_i)^\top - I} \leq \sigma^2 \tO (\eta)
\end{equation}

To derive the bounds, we proceed as follows:

\begin{enumerate}
    \item Firstly in the analysis alone, we will condition on the event that $\abs{\inp{X_i}{\Delta}} \leq O(\sqrt{\log 1 / \epsilon})$ where $\Delta = \frac{w^*}{\norm{w^*}}$ and $\abs{\epsilon_i} \leq O(\sqrt{\log 1 / \epsilon})$. 
    
    
    
    \item Conditioned on the event, we then show that for any set of $1 - O(\eta)$ points the two conditions hold.
    
    \item The proof of the first condition is identical to the proof in the previous case except we need a tighter lower bound (We need deviation $\tO(\eta)$ here instead of $O(\sqrt{\eta})$). \Enote{The proof is exactly the same; except in the place where Cauchy-Schwartz was used, the tail bound needs to be updated from simple Chebyshev to the sub-exponential tail bound, which gives a $O(e^{-1/\sqrt{\eta}})$ for that step; the following step "fixes" that to $O(\eta)$ } \Ynote{Yeah. It's very similar but you'd need a tighter bound on the deviation. Shouldn't be too hard.}
    
    \item For the second term, we perform the following decomposition:
    
    \begin{equation*}
        Y_i^2 X_iX_i^\top = \inp{X_i}{w^*}^2 X_iX_i^\top + 2 \epsilon_i \inp{X_i}{w^*} X_i X_i^\top + \epsilon_i^2 X_i X_i^\top
    \end{equation*}
    
    \Enote{The middle term should be a plus right? Not that it remotely matters or affects anything} \Ynote{Noted}
    
    and the proceed to bound the spectral norm of any $O(\eta)$ fraction of the vectors for each of them. Similar to the gridding arguments of the previous parts but easier as we wouldn't need to truncate again as the scalars are already sub-gaussian. We could Cauchy Schwarz the middle term so as to deal only with the first and last ones. $\mc{R} - \text{Removed set}$
    
    \begin{align*}
        &\sum_{i \in \mc{R}} \lprp{\inp{X_i}{w^*}^2 X_iX_i^\top + 2\epsilon_i \inp{X_i}{w^*} X_iX_i^\top + \epsilon_i^2 X_iX_i^\top} \text{ Pick Direction $u$} \\
        &\sum_{i \in \mc{R}} \lprp{\inp{X_i}{w^*}^2 \inp{X_i}{u}^2 + 2\epsilon_i \inp{X_i}{w^*} \inp{X_i}{u}^2 + \epsilon_i^2 \inp{X_i}{u}^2} \\
        &\leq \sum_{i \in \mc{R}} 2 (\inp{X_i}{w^*}^2 \inp{X_i}{u}^2 + \epsilon_i^2 \inp{X_i}{u}^2) \leq \tO(\eta) n
    \end{align*}
\end{enumerate}

\subsection{To Do: Algorithm Proofs}

The main steps left in the proof are the following:

\begin{enumerate}
    \item Prove that one can obtain good primal weights efficiently.
    \item Prove that primal approximation gives good estimate of the gradient.
    \item Conclude the gradient descent proof.
    
    \item Extra step for the sub-gaussian case and how to solve it efficiently. \Ynote{I'll take this}
\end{enumerate}

Notation:
\begin{equation*}
    \mb{E}_S [X_i] = \abs{S}^{-1} \sum_{i \in S} X_i \text{ and } \mb{E}_s [X_i] = \sum_{i = 1}^n s_i X_i.
\end{equation*}

The lemma for the first part would look like this
\begin{lemma}
    \label{lem:htprimtemp}
    Assume the deterministic conditions guaranteed by \cref{lem:htdet}. Given $w$, produce in time $\tO(nd / poly(\epsilon))$, a set of primal weights $0 \leq s_i \leq 1 / ((1 - 10\eta)n)$ such that:
    \begin{equation*}
      \lmax{ \mb{E}_s [G_i(w)G_i(w)^\top]} \leq O(1) \cdot \lprp{\norm{w - w^*}^2 + \sigma^2}.
    \end{equation*}
\end{lemma}

\begin{proof}  
    The rough proof would go like this. Look at the $(1 - 5\eta)n$ closest points to $0$. The mean of squared distances will give you an upper bound like $d (\norm{w - w^*}^2 + \sigma^2)$. Now, do $O(\log d)$ steps where you keep halfing the value used as $1 / \rho$ in Ilias' packing covering solvers (As long as $\norm{s} \geq 1 - \eta / 100$ or something).
\end{proof}

The lemma for the second part
\begin{lemma}
    \label{lem:htgapxtemp}
    Given a solution from \cref{lem:htprimtemp}, $s$, we have:
    \begin{equation*}
        \norm{\mb{E}_s [G_i(w)] - G^*{w}} \leq \sqrt{\eta} O(1) \cdot \lprp{\norm{w - w^*} + \sigma}.
    \end{equation*}
\end{lemma}

With the previous two lemmas, a straightforward gradient descent proof should give the theorem for the heavy tailed case. We get $O(\sqrt{\eta})$ error with $O(d / \eta)$ samples.

Finally, we have an adjustment step for the gaussian case. Solving it efficiently is a bit more of a pain. The main lemma would look like this:

\begin{lemma}
    \label{lem:sgfintemp}
    Assume conclusions of \cref{lem:sgdet}. Then, we can obtain in time $\tO(nd / poly(\eta))$, a set of primal weight $0 \leq s_i \leq 1 / (1 - 10\eta)n$ such that:
    \begin{equation*}
        \mb{E}_s [G_i(w) G_i(w)^\top] \preccurlyeq \sigma^2 \cdot I + O(1) \cdot \sigma^2 \eta \log^2 1 / \eta.
    \end{equation*}
\end{lemma}
\Ninote{Remark the difference with the heavy tailed case where we are happy to solve the sdp up to any multiplicative constant }    

\begin{proof}
   \Ynote{Note that in both proofs, only the upper bound is important. Estimate $\sigma$ from $\abs{Y_i}^2$ (Truncated mean for example.) or look at the lengths of $Y_i X_i$. And now binary search over $1 / \rho$ in Ilias' SDP solver for $O(\log d / \eta)$ times till you get a upper bound which satisfies our requirements. This should prove the first part. The second part is an argument very similar to the heavy tailed gradient estimation step except you have to be a little bit more careful. You should account for the fact that $1$ variance already exists in the good $X_i$. }
\Ninote{We should emphasize the proof is very close to the one of Proposition 4.1 in Ilias paper, }    
    
We first estimate the value of the variance $\sigma$ by robustly estimate the mean of $Y_i^2$ which is $\bbE[Y_i^2]=\sigma^2+\norm{w^*}^2$. Since $\norm{w^*}=O(\sqrt{\eta})$ by \cref{as:sgiest}, we obtain an estimate $\hat \sigma$ such that $|\sigma-\hat\sigma|=O(\sqrt{\eta})$. 
    
We proceed as in the proof of \cref{lem:htprimtemp}.  We first solve the packing SDP~\ref{eq:sdppack} for $\rho=1/\tilde \sigma^2$. If   $\normo{\tilde s}\geq (1-\eta/2)$, then we can convert this solution into a solution of the SDP~\eqref{eq:primalsdp} with parameter $10\eta$ whose objective value is at most $\frac{\tilde \sigma^2}{1-\eta/2}= \sigma^2(1+O(\eta))$. Therefore we assume now that $\OPT_{\rho=1/\tilde \sigma^2}<1-\eta/3$.
    
Let us define $\rho_1$ such that  $\OPT_{\rho_1}=1-\eta/3$,  we want to find a suitable value of $\rho$ such that $\rho\in[\rho_*,\rho_1]$. If we approximately solve the packing SDP~\ref{eq:sdppack} for this $\rho$ up to a multiplicative error $1+O(\eta)$, we obtain a weight vector $\tilde s$ such that $\normo{\tilde s}\geq (1-O(\eta)))\OPT_{\rho}\geq (1-O(\eta)))\OPT_{\rho_1}\geq 1-\eta/2$---since $\OPT_\rho$ is non-increasing in $\rho$. Therefore, applying \cref{lem:timepack}, we can construct a primal solution $s$ of the SDP~\eqref{eq:primalsdp} with parameter $10\eta$ whose objective value is at most $\frac{\rho_*}{1-\eta/2}= \sigma^2+O(\eta)$.
    
We find such $\rho$ by binary search; decreasing the value of $\rho$ if $\normo{\tilde s}<1-\eta/3$ and increasing it if $\normo{\tilde s}>1$. To bound the running time of this procedure, we first note the length of the interval $[\rho_*,\rho_1]$ is bounded by $\eta\rho_*=\eta/\sigma^2$. Indeed $\rho_*\geq(1-\eta/4)\rho_1$ (using \cref{lem:optpack}, we obtain otherwise $1-\eta/3=\OPT_{\rho_1}\geq (1-\eta/4)\OPT_{\rho_*}=(1-\eta/4)$) and $\rho_1-\rho_*\geq \eta/4\rho_1\geq \eta \rho_*/4 $. Thus this procedure requires $\log(\eta)$ step since we start from a interval length of $1/\tilde \sigma^2$ and the target interval is of length $\eta/\sigma^2$.
    
We conclude as in the proof of \cref{lem:htprimtemp} that the total running time is 
    \[O(\log(\eta))\cdot O(\log\log(\eta))\cdot\tilde O(Nd/\eta^6).
    \]
\end{proof}

\begin{lemma}
    \label{lem:sgfintemp2}
    Assume the deterministic conditions guaranteed by \cref{lem:sgdet}. Then given a solution, $s$, satisfying:
    \begin{equation*}
        \lambda_{\max}\lprp{\mb{E}_s [G_i G_i^\top]} \leq \sigma^2 + O(1) \cdot \sigma^2 \eta \log^2 1 / \eta
    \end{equation*}
    we have $\norm{\mb{E}_s [G_i - w^*]} \leq O(1) \cdot \sigma \eta \log 1 / \eta$.
\end{lemma}
\begin{proof}
    We begin by decomposing $s$ as $s = \sum_{\alpha \in \mc{E}_{6\eta}} \gamma_\alpha \alpha$ by \cref{lem:extpts} with $\sum_{\alpha \in \mc{E}_{6\eta}} \gamma_\alpha = 1$. Finally, we define $\alpha_T = \sum_{i \in T} \alpha_i$. Now, we have:
    \begin{equation*}
        \norm{\sum_{i = 1}^n s_i G_i - w^*} \leq \norm{\sum_{i \in S} s_i (G_i - w^*)} + \norm{\sum_{i \notin S} s_i (G_i - w^*)}.
    \end{equation*}
    We bound the first term as follows:
    \begin{align*}
        \norm{\sum_{i \in S} s_i (G_i - w^*)} \leq \sum_{\alpha \in \mc{E}_{6\eta}} \gamma_\alpha \norm{\sum_{i \in S} \alpha_i (G_i - w^*)} = \sum_{\alpha \in \mc{E}_{6\eta}} \gamma_\alpha \cdot \frac{1}{\alpha_S} \norm{\mb{E}_{\text{Supp}(\alpha) \cap S} (G_i - w^*)} \leq O(1)\cdot \sigma \eta \log 1 / \eta
    \end{align*}
    where the last inequality follows because we have $\text{Supp}(\alpha) \cap [n] \geq (1 - 10\eta)n$ and from \cref{lem:sgdet}. For the second term, we have for all $\norm{u} = 1$:
    \begin{align*}
        \mb{E}_s [\inp{u}{(G_i - w^*)} \bm{1} \lbrb{i \notin S}] &\leq (\mb{E}_s [\inp{u}{G_i - w^*}^2 \bm{1} \lbrb{i \notin S}])^{1/2} (\mb{E}_s [\bm{1} \lbrb{i \notin S}])^{1/2} \\
        &\leq 2 \sqrt{\eta} (\mb{E}_s [\inp{u}{G_i - w^*}^2 \bm{1} \lbrb{i \notin S}])^{1/2}\\
        &\leq 4\sqrt{\eta} (\mb{E}_s [\inp{u}{G_i }^2 \bm{1} \lbrb{i \notin S}])^{1/2} + 4\sqrt{\eta} (\mb{E}_s [\inp{u}{w^*}^2 \bm{1} \lbrb{i \notin S}])^{1/2}
    \end{align*}
    We finally bound the last terms in the above display as follows:
           \begin{align*}
        \mb{E}_s [\inp{u}{G_i }^2 \bm{1} \lbrb{i \notin S}] &= \mb{E}_s [\inp{u}{G_i }^2] - \mb{E}_s [\inp{u}{G_i }^2 \bm{1} \lbrb{i \in S}] \\
        &\leq (1 + O(1) \eta \log^2 1 / \eta) \sigma^2 - \sum_{\alpha \in \mc{E}_{6\eta}} \gamma_\alpha \cdot \alpha_S \cdot \mb{E}_{\text{Supp} \cap S} [\inp{u}{G_i - w^*}^2 \bm{1} \lbrb{i \in S}] \\
        &\leq \sigma^2 \lprp{1 + O(1) \eta \log^2 1 / \eta -(1 - O(1) \cdot \eta \log^2 1 / \eta)} \leq O(1)\cdot \sigma^2 \eta \log^2 1 / \eta
    \end{align*}
    where the last inequality follows from \cref{lem:extpts,lem:sgdet}. And 
    \[
        \mb{E}_s [\inp{u}{w^* }^2 \bm{1} \lbrb{i \notin S}] \leq\norm{w_*}^2   \mb{E}_s [\bm{1} \lbrb{i \notin S}]\leq 4\eta \norm{w_*}^2\leq 4\eta^{3/2},
    \]
    where the last inequality follows from  \cref{as:sgiest}.   Substituting the above bounds in the previous equations, we conclude the proof of the lemma.
\end{proof}

==> content/preliminaries.tex <==
\section{Preliminaries}



==> content/regression.tex <==
\section{Regression}


==> content/sg_summary.tex <==
\subsection{Sub-gaussian Concentration}
\label{sec:sgconc}
\Nnote{@ Efe can you state the main lemma and say you focus on the second moment here and explain the main terms that are different then HT case?}

In this section we prove concentration results pertaining to the case where the random variables, $X$ and $\epsilon$ are sub-Gaussian instead of the much milder L4-L2 assumptions we had previously considered. This allows us to obtain much tighter bounds on the recovery error than those obtained in Section~\ref{sec:htconc}. \Ninote{Do you really meant recovery error?} In particular, we can show that, assuming one has a fairly good ($O(\sqrt{\eta})$) estimate of the mean, the robust mean of the gradient evaluated at that point is (w.h.p.) a very accurate estimate of the difference of the mean ($O(\eta)$) \Ynote{We should be more precise here.}. 

\Ynote{The following results also require \cref{as:sgiest}} More formally, to be able to run the robust mean estimation algorithm, we want to show that the following theorem holds:

\begin{lemma}
    \label{lem:sgdet}
    Let $\mc{D}$ satisfy \cref{as:sgassump}. Then, given $n = \tO (d / \eta^2)$ $2\eta$-corrupted samples from $\mc{D}$, we have with probability at least $1 - 1 / d^2$, there exists a set $S \subset [n]$ with $\abs{S} \geq (1 - 3\eta)n$ such that for any $T \subset S$ with $\abs{T} \geq (1 - 10\eta)n$:
    \begin{equation*}
        \norm{\mb{E}_T [Y_i X_i] - w^*} \leq C_1 \sigma \eta \log{1 / \eta} \text{ and } \norm{\mb{E}_T [Y_i^2 X_i X_i^\top] - \sigma^2 \cdot I} \leq C_2 \sigma^2 \eta \log^2 1 / \eta.
    \end{equation*}
    Furthermore, for all $i \in S$, we have $\norm{Y_i X_i} \leq C_3 \sigma \sqrt{\log 1 / \eta} (\sqrt{d} + \sqrt{\log 1 / \eta})$ for some absolute constants $C_1, C_2, C_3$
\end{lemma}

To show that this theorem holds for some set $S$, we will create a desirable, high probability set $\mc{H}$ that essentially allows us to treat the samples and the noise as bounded. 


To see why one might expect this theorem to hold, we can look at the gradient more carefully:

 \begin{equation*}
        G_i = Y_i X_i = \inp{X_i}{(w^* - w^\dagger)} X_i + \epsilon_i X_i 
\end{equation*}

Now, we note that the expectation of the gradient is simply $(w^* - w^\dagger)$, since $X_i$ has identity covariance, and $\epsilon_i$ is mean 0 and independent of $X_i$. Furthermore, since $X_i$s are subgaussian, we can claim that with high probability the (uncorrupted) $X_i$s are in a ball of radius $\sqrt{d}$ around the original mean, which means we can control the size of the deviations in this expression quite well. In particular, we explicitly control the behavior of the $\epsilon_i X_i$ term formally in the following lemma:

\begin{lemma}
    \label{lem:sgerrconcmean}
    Let $\mc{D}$ satisfy \cref{as:sgassump}. Then for $n = \tO (d / \eta^2)$ samples from $\mc{D}$, we have with probability at least $1 - 3 / (10d^2)$, for any set $S \subset [n]$ with $\abs{S} \geq (1 - 10\eta)n$, we have:
    
    \begin{equation*}
       \norm*{ \sum_{i \in S} \frac{Z_i}{n}} \leq C \sigma \eta \log 1 / \eta
    \end{equation*}
    
    for some absolute constant C, where $Z_i = \epsilon_i X_i\bm{1} \lbrb{(\epsilon_i, X_i) \in \mc{H}}$ 
     
\end{lemma}

The trickier part is to analyze the second order condition required for the success of the \cref{alg:sgalg}, so we start by expanding out what the second order term looks like:

 \begin{equation*}
        G_i G_i^\top = \inp{X_i}{(w^* - w^\dagger)}^2 X_iX_i^\top + 2\epsilon_i \inp{X_i}{w^*} X_i X_i^\top + \epsilon_i^2 X_iX_i^\top.
\end{equation*}

We note that this lemma requires the control of three terms:

\begin{itemize}
    \item For the $\inp{X_i}{(w^* - w^\dagger)}^2 X_iX_i^\top$ term, we rely on the fact that our current estimate is accurate up to $\sqrt{\eta}$ error, and so we can show that this term has to be of order $O(\sigma^2 \eta)$ by concentration results.
    
    \item The middle term $\epsilon_i \inp{X_i}{(w^* - w^\dagger)} X_i X_i^\top$ has expectation 0 by the expectation of the noise, and the inner product is small with high probability. While this term is hard to control for individual samples, on average, we can show that the samples we don't choose cannot influence the size of this sum too much.        
    
    \item We note that the term $\epsilon_i^2 X_iX_i^\top$ has expectation $\sigma^2 I$ by moment assumptions, and by standard concentration results, we can show that it does not deviate too much from its expectation: 
     
    \begin{lemma}
    \label{lem:sgerrconcvar}
    Let $\mc{D}$ satisfy \cref{as:sgassump}. Then for $n = \tO (d / \eta^2)$samples from $\mc{D}$, we have with probability at least $1 - 3d^2 / 10$, for any set $S \subset [n]$ with $\abs{S} \geq (1 - 10\eta)n$, we have:
    \begin{equation*}
        \norm*{\sum_{i \in S} \frac{Z_iZ_i^\top}{n} - \sigma^2 I} \leq C \sigma^2 \eta \log^2 1 / \eta
    \end{equation*}
    
     where $Z_i = \epsilon_i X_i\bm{1} \lbrb{(\epsilon_i, X_i) \in \mc{H}}$ for some absolute constant $C$.
     
    \end{lemma}
    
\end{itemize}

Combining the results above, we get the following lemma which controls the second moment of the gradient in a high probability set $\mc{H}$:
\begin{lemma}
    \label{lem:sgcovconc}
    Let $\mc{D}$ satisfy \cref{as:sgassump,as:sgiest}. Then for $n = \tO (d / \eta^2)$, we have with probability at least $1 - 1 / (2d^2)$, that for any $S \subset [n]$ with $\abs{S} \geq (1 - 10\eta)n$:
    \begin{equation*}
        \norm*{n^{-1} \sum_{i \in S} G_i G_i^\top \bm{1} \lbrb{(X_i, \epsilon_i) \in \mc{H}} - \sigma^2 \cdot I} \leq C \eta \log^2 1 / \eta \sigma^2.
    \end{equation*}
    for some absolute constant C
\end{lemma}

Finally, to go from this lemma to \cref{lem:sgdet}, we note that because our set $\mc{H}$ had a high probability, with high probability, most of our samples will fall in it, and so we can simply pick the elements to plug in the lemmas above to be those ones, which now gives a deterministic guarantee with high probability.  

% From \ref{lem:htmeanconc} \Ynote{Theorem for Heavy Tailed case}, we can assume that we have an initial estimate $w$ such that $(w - w^*) \leq O(\sqrt{\eta})$. Therefore, by subtracting out $\inp{X_i}{w}$ from all the data points, our problem reduces to a setting where we additionally have $\norm{w^*} \leq O(\sqrt{\eta})$. We make this formal in the following assumption:
% \begin{assumption}
%     \label{as:sgiest}
%     We assume that there exists a constant $\nu$, such that $\norm{w^*} \leq \nu \sigma \sqrt{\eta}$.
% \end{assumption}
% Note, that under \cref{as:sgassump}, we have $\mb{E} [\norm{X}] \leq \lprp{\mb{E} [\norm{X}^2]}^{1/2} = \sqrt{d}$. Throughout the analysis we refer at several points to the following events:
% \begin{gather*}
%     \mc{H}_{\epsilon} = \{\abs{\epsilon_i} \leq 6 \phi \sqrt{\log 1 / \eta}\} \\ 
%     \mc{H}_{l} = \{\norm{X} \leq 7\psi \sqrt{d} + 24 \psi \sqrt{\log 1 / \eta}\} \\
%     \mc{H}_{o} = \{\abs{\inp{X}{w - w^*}} \leq 6 \psi \norm{w - w^*} \sqrt{\log 1 / \eta}\}
% \end{gather*}
% Note, that from \cref{lem:sgmeanconc} the event, $\mc{H} = \mc{H}_{\epsilon} \cap \mc{H}_l \cap \mc{H}_o$ occurs with probability at least $1 - \eta^{16}$. We start by proving a lemma pertaining to the noise terms arising in the gradient.
% \begin{lemma}
%     \label{lem:sgerrconc}
%     Let $\mc{D}$ satisfy \cref{as:sgassump}. Then for $n = \tO (d / \eta^2)$samples from $\mc{D}$, we have with probability at least $1 - 3d^2 / 10$, for any set $S \subset [n]$ with $\abs{S} \geq (1 - 10\eta)n$, we have:
%     \begin{equation*}
%       \norm*{ \sum_{i \in S} \frac{Z_i}{n}} \leq O(\sigma \eta \log 1 / \eta) \text{ and } \norm*{\sum_{i \in S} \frac{Z_iZ_i^\top}{n} - \sigma^2 I} \leq O(\sigma^2 \eta \log^2 1 / \eta)
%     \end{equation*}
    
%      where $Z_i = \epsilon_i X_i\bm{1} \lbrb{(\epsilon_i, X_i) \in \mc{H}}$.
% \end{lemma}
% \begin{proof}
% (Sketch) 

% We quickly note that the upper bound on the operator norm of the sum $Z_i Z_i^\top$ is easier since discarding samples simply reduces the operator norm, so the high probability bound follows from using Bernstein on the whole sample set. 

% So, the hard part is to prove the lower bound for the operator norm inequality, and for that, we use a standard gridding argument. We observe that for a given index $i$, and a vector $u$, with high probability, $\inp{u}{X_i}^2 $ is $O(\log1/\eta)$. and since by the definition of $\mc{H}$, the samples are truncated, we can use Hoeffding inequality to prove a concentration result for the behavior of the inner product. Thus, after a union bound, and noting that removing a small amount of bounded samples does not change the average too much, the result follows.   

% To control the norm of the sum of $Z_i$, we note that $Z_i$ is a subgaussian when restricted to the event $\mc{H}$ since $\epsilon_i$ is bounded in this set. Now, the result follows from the first operator bound.

% \end{proof}

% In the following lemma, we prove that for all sufficiently large sets of data points whose gradients have well behaved covariance structure.

% \begin{lemma}
%     \label{lem:sgcovconc}
%     Let $\mc{D}$ satisfy \cref{as:sgassump,as:sgiest}. Then for $n = \tO (d / \eta^2)$, we have with probability at least $1 - 1 / (2d^2)$, that for any $S \subset [n]$ with $\abs{S} \geq (1 - 10\eta)n$:
%     \begin{equation*}
%         \norm*{n^{-1} \sum_{i \in S} G_i G_i^\top \bm{1} \lbrb{(X_i, \epsilon_i) \in \mc{H}} - \sigma^2 \cdot I} \leq O(\eta \log^2 1 / \eta))\sigma^2.
%     \end{equation*}
% \end{lemma}
% \begin{proof}
%     We first explicitly write out the expression for $G_i G_i^\top$ as follows:
%     \begin{equation*}
%         G_i G_i^\top = \inp{X_i}{w^*}^2 X_iX_i^\top + 2\epsilon_i \inp{X_i}{w^*} X_i X_i^\top + \epsilon_i^2 X_iX_i^\top.
%     \end{equation*}
    
%     Since we are using a sufficiently accurate $w^*$, the first term is essentially controlled by the behaviour of $X_iX_i^\top$ since $\inp{X_i}{w^*}^2$ is bounded, which can be controlled by matrix Bernstein as in $\cref{lem:sgerrconc}$. The last term can be controlled by focusing on the event of $\cref{lem:sgerrconc}$. The middle term is very similar to the last term where we rely on the $\epsilon_i$ being bounded, and then check the maximum possible deviation a bounded set of elements can cause. 
    
    
% \end{proof}


% We now present the main result of this section which establishes the deterministic conditions required for the success of \cref{alg:sgalg}. 

% \begin{lemma}
%     \label{lem:sgdet}
%     Let $\mc{D}$ satisfy \cref{as:sgassump,as:sgiest}. Then, given $n = \tO (d / \eta^2)$ $2\eta$-corrupted samples from $\mc{D}$, we have with probability at least $1 - 1 / d^2$, there exists a set $S \subset [n]$ with $\abs{S} \geq (1 - 3\eta)n$ such that for any $T \subset S$ with $\abs{T} \geq (1 - 10\eta)n$:
%     \begin{equation*}
%         \norm{\mb{E}_T [Y_i X_i] - w^*} \leq O(1) \sigma \eta \log{1 / \eta} \text{ and } \norm{\mb{E}_T [Y_i^2 X_i X_i^\top] - \sigma^2 \cdot I} \leq O(1) \cdot \sigma^2 \eta \log^2 1 / \eta.
%     \end{equation*}
%     Furthermore, for all $i \in S$, we have $\norm{Y_i X_i} \leq O(1)\cdot \sigma \sqrt{\log 1 / \eta} (\sqrt{d} + \sqrt{\log 1 / \eta})$.
% \end{lemma}
% \begin{proof}
%     Assume that the conclusions of \cref{lem:sgerrconc,lem:sgcovconc,lem:sgmeanconc}. This happens by the union bound with probability at least $1 - 9/(10d^2)$. Now, consider the set $S' = \{i: (X_i, \epsilon_i) \in \mc{H}\}$. Since, we have $\mb{P} ((X_i, \epsilon_i) \notin \mc{H}) \leq \eta^{16}$, we have via the Bernstein bound that with probability at least $1 - d^2/10$ that $\abs{S'} \geq (1 - \eta)n$. Now, since we have $2\eta n$ adversarial corruptions at least $(1 - 3\eta)n$ points of $S'$ are not corrupted. Let $S$ be the uncorrupted points of $S'$. This proves the final claim of the lemma.
    
%     Let $T \subset S$ with $\abs{T} \geq (1 - 10\eta)n$. The second claim now follows from the conclusion of \cref{lem:sgcovconc}. The first term claim now follows from \cref{lem:sgmeanconc,lem:sgerrconc} as:
%     \begin{equation*}
%         \norm{\mb{E}_T [G_i] - w^*} \leq \norm{(\mb{E}_T [X_iX_i^\top] - I)w^*} + \norm{\mb{E}_T [\epsilon_i X_i]} \leq O(1) \cdot \sigma \eta \log 1 / \eta.
%     \end{equation*}
%     This concludes the proof of the lemma.
% \end{proof}

==> content/techniques.tex <==
\section{Lemmas}




\begin{lemma}
    Distance Estimation Lemma
\end{lemma}

\begin{lemma}
    Gradient Estimation Lemma
\end{lemma}



==> content/warm.tex <==
\section{Analysis warm-up} 
We observe data $(X_j,Y_j)$. We th We will consider at point $w$ the gradient estimate $G_i$ of the ith bucket defined as $G_i (w)= \bm{X}_i^\top(\bm{X}_iw - \bm{Y}_i)= \hat \Sigma_i(w-w_*) - X_i\eta_i$.
\begin{gather*}
  \max \sum_{i = 1}^{k} b_i \\
  b_i^2 = b_i \\
  \norm{v}^2 = 1 \\
  b_i \inp{v}{G_i(w)} \geq b_i^2 r \quad \forall i \in [k] \label{eq:mte} \tag{\textbf{MTE}}
\end{gather*}

We define the affine operator $G(w)$ as follows:

\begin{equation*}
    G(w) := \tSigma (w - w^*), \qquad \tSigma := \frac{\mb{E}_{X, y} [XX^\top \cdot \bm{1} \{\norm{X} \leq \alpha\}]}{\mb{P} [\norm{X} \leq \alpha]}
\end{equation*}
In the proofs of our lemmas relating to the correctness of the Distance Estimation and the Gradient Estimation steps, we make use of the following assumption:
\begin{assumption}
    \label{as:exact}
    For the bucket means, $\bm{G} = (G_1, \dots, G_k)$, we have for any $w$:
    \begin{equation*}
        \forall t\geq 1, \forall v \in \mb{R}^{d}, \norm{v} = 1 \;\Rightarrow \abs*{\{i: \inp{G_i(w) - G(w)}{v} \geq A_1+A_2 \norm{w - w_*}_\Sigma\}} \leq 0.05k
    \end{equation*}
\end{assumption}
The assumption is a formalization of the insight of \citep{lugosi2017sub}, which shows that along all directions, $v$, most of the bucket means are within a small radius of the true mean, $\mu$, with high probability\footnote{This will be made precise in Corollary~\ref{cor:dconce}.}.

First, we prove that the \textbf{Distance Estimation} step defined in Algorithm~\ref{alg:deste} is correct.

\begin{lemma}
  \label{lem:deste}
Suppose Assumption~\ref{as:exact} holds and let $w \in \mathbb{R}^d$. Then the output, $d^*$, of Algorithm~\ref{alg:deste} with inputs $\bm{Z}$ and $w$ satisfies:
  \begin{equation*}
    \big\vert d^* - \norm{G(w)} \big\vert \leq \rade{}.
  \end{equation*}
\end{lemma}
\begin{proof}
  Let $r^* = \rade{t}$. We first prove the lower bound $\norm{\Gt{t}}-r^*\leq \dt{t}$. We may assume that $\norm{\Gt{t}} > r^*$, as the alternate case is trivially true. For $r = \norm{\Gt{t}} - r^*$, we can simply pick the vector $v = \dd$ where $\dd$ is the unit vector in the direction of $\Gt{t}$. Under Assumption~\ref{as:exact}, we have that for at least $0.95k$ points:
    \begin{equation*}
      \inp{G_i}{v} = \inp{G_i - \Gt{t}}{v} + \inp{\Gt{t}}{v} \geq \norm{\Gt{t}} - r^* = r.
    \end{equation*}
  This implies the lower bound holds in the case where $\norm{\xt{t} - \mu} > r^*$.

For the upper bound $\dt{t}\leq \norm{\Gt{t} }+r^* $, suppose, for the sake of contradiction, there is a value of $r >\norm{\Gt{t}}+r^*$ for which the optimal value of $\mte(\xt{t},r,\bm{G})$ is greater than $0.9k$. Let $v$ be the solution of $\mte(\xt{t},r,\bm{G})$. This means that for $0.9k$ of the $G_i$, we have:

  \begin{equation*}
    \inp{G_i-\Gt{t}}{v} = \inp{G_i}{v} - \inp{\Gt{t} }{v} \geq r - \norm{\Gt{t}} > r^*.
  \end{equation*}
  This contradicts Assumption~\ref{as:exact} and proves the upper bound.
\end{proof}
Next, we prove the correctness of the \textbf{Gradient Estimation} step from Algorithm~\ref{alg:geste}.
\begin{lemma}
  \label{lem:geste}
  Suppose Assumption~\ref{as:exact} holds and $w$ satisfies:
  \begin{equation}\label{eq:assummu}
    \norm{\Gt{}} \geq \radae{},
  \end{equation}
and let $\dd$ denote the unit vector in the direction of $\Gt{}$. Then, we have that the output of Algorithm~\ref{alg:geste}, $g$, with inputs $\bm{Z}$ and $w$ satisfies:
  \begin{equation*}
    \inp{\vt{}}{\dd} \geq \frac{1}{2}.
  \end{equation*}
\end{lemma}
\begin{proof}
  Let $r^* = \rade{t}$.  We have, from the definition of $\dt{t}$, that for $0.9k$ of the $G_i$,     \mbox{$\inp{G_i - \xt{t}}{\vt{t}} \geq \dt{t}$}.
  We also have, under Assumption~\ref{as:exact}, that
  $
    \inp{G_i-\Gt{t} }{\vt{t}} \leq r^*
  $ for $0.95k$ of the $G_i$.
  From the pigeonhole principle, there exists a $G_j$ which satisfies both those inequalities. Therefore, for that $G_j$, the lower bound from Lemma~\ref{lem:deste} implies
  \begin{equation*}
    \norm{\Gt{t}} - r^* \leq \dt{t} \leq \inp {G_j} {\vt{t}} = \inp{G_j - \Gt{t}}{\vt{t}} + \inp{ \Gt{t}}{\vt{t}} \leq r^* + \norm{ \Gt{t}}\inp{\dd}{\vt{t}}.
  \end{equation*}
  By rearranging the above inequality and using the assumption on $\norm{\mu - \xt{t}}$ in \eq{assummu},
  we get the required conclusion.
\end{proof}
To control the probability that Assumption~\ref{as:exact} holds, we assume the correctness of the following corollary of Lemma~\ref{lem:mnConc}, formalizing the insight of \citep{lugosi2017sub}:
\begin{corollary}
\label{cor:dconce}
Let $\bm{Y} = (Y_1, \dots, Y_k) \in \mb{R}^{k \times d}$ be $k$ i.i.d.~random vectors with mean $\mu$ and covariance $\Lambda$. Furthermore, assume $k \geq \nbu$. Then we have for all $v\in \mb{R^d}$ such that $\Vert v\Vert=1$:
\begin{equation*}
 \abs*{\{i: \inp{Y_i - \mu}{v} \geq \rady\}} \leq 0.05k{}
\end{equation*}
{}
with probability at least $1 - \delta$.

\end{corollary}
By instantiating Corollary~\ref{cor:dconce} with the $Y_i = Z_i$, we see that Assumption~\ref{as:exact} holds with high probability. 

Finally, we put the results of Lemma~\ref{lem:deste}, Lemma~\ref{lem:geste} and Corollary~\ref{cor:dconce} together to prove Theorem~\ref{thm:sgmeste}.

\begin{proof}
%[of Theorem~\ref{thm:sgmeste}]
  Assume first that Assumption~\ref{as:exact} holds. Let $r^* = \radae{t}$. To start with, let us define the set ${\mathcal{G} = \{w: \norm{w - \wstar}_{\Sigma^2} \leq r^*\}}$. We prove the theorem in two cases:
  \begin{enumerate}
    \item[] \textbf{Case 1: } None of the iterates $x_t$ lie in $\mathcal{G}$. In this case, note that by Lemma~\ref{lem:deste} and the definition of $r^*$, we have:
    \begin{equation}
    \label{eq:dbe}
        \frac{3}{4} \norm{\xt{t} - \mu}_{\Sigma^2} \leq \dt{t} \leq \frac{5}{4} \norm{\xt{t} - \mu}_{\Sigma^2}.
    \end{equation}
    Moreover, we have by the definition of the update rule of $x_t$ in Algorithm~\ref{alg:meste}:
    \begin{align*}
      \norm{\xt{t + 1} - \wstar}_\Sigma^2 &= \norm{\xt{t} - \wstar}_\Sigma^2 - \frac{1}{2} \dt{t} \inp{\Sigma(\xt{t} - \wstar)}{\vt{t}} + \frac{\dt{t}^2\norm{\Sigma}^2}{16} \leq \norm{\xt{t} - \mu}_\Sigma^2 - \frac{\dt{t} \norm{\xt{t} - \wstar}_{\Sigma^2}}{4} + \frac{\dt{t}^2\norm{\Sigma}^2}{16} \\
      &\leq \norm{\xt{t} - \wstar}_\Sigma^2 - \frac{3}{16} \norm{\xt{t} - \wstar}_{\Sigma^2}^2 + \frac{25\norm{\Sigma}^2}{256} \norm{\xt{t} - \wstar}_{\Sigma^2}^2 \leq \frac{23}{25} \norm{\xt{t} - \mu}^2,
    \end{align*}
    where we have used Lemma~\ref{lem:geste} for the first inequality and the inequalities in \eqref{eq:dbe} for the second inequality. By iteratively applying the above inequality, we get the conclusion of the theorem in this case. 
    \item[] \textbf{Case 2: } At least one of the iterates $\xt{t}$ lies in $\mathcal{G}$. For this iterate, 
    \[
  \mu  \norm{\xt{{t}} - \wstar}_{\Sigma} \leq  \norm{\xt{{t}} - \wstar}_{\Sigma^2} \leq 4A_1+4A_2 \norm{\xt{{t}} - \wstar}_{\Sigma},
    \]
    and $ \norm{\xt{{t}} - \wstar}_{\Sigma} \leq \frac{4A_1}{\mu-4A_2}$.
    Therefore, we have from Lemma~\ref{lem:deste}:
    \begin{equation*}
      \dt{t} \leq \gpdbe{t}.
    \end{equation*}
    We also have at the completion of the algorithm, from another application of Lemma~\ref{lem:deste}:
    \begin{equation*}
      \norm{\xt{{t_0}} - \wstar}_{\Sigma^2} - (\rade{{t_0}}) \leq \optd \leq \dt{t} \leq  \gpdbe{t}\leq 5A_1 +\frac{20A_1A_2}{\mu-4A_2}.
    \end{equation*}
      By re-arranging the above inequality, we get 
      \[
      \norm{\xt{{t_0}} - \wstar}_{\Sigma} \leq \frac{2A_1}{\mu-A_2}[ 3 +\frac{10A_2}{\mu-4A_2}]
      \]
      
      the desired result.
  \end{enumerate}
  By Corollary~\ref{cor:dconce}, Assumption~\ref{as:exact} holds with probability at least $1-\delta$ and therefore, the conclusions from Case 1 and Case 2 hold with probability $1-\delta$. 
\end{proof}
Bearing in mind that the polynomial optimization problem \ref{eq:mte} is non-convex, we consider a convex relaxation in the following section.  





\begin{assumption}
For $0.9K$ buckets $$| u^\top (\hat{\Sigma}_i - \Sigma) u | \leq C(\kappa) u^\top \Sigma u $$ holds
\end{assumption}

\begin{corollary}
Let $\Delta = w_* - w_t $ Then, for the same buckets, 
$$|\Delta^\top (\hat{\Sigma}_i - \Sigma) v| \leq O(C(\kappa) \sqrt{\norm{\Sigma}} \norm{\Delta}_\Sigma) $$ %where $\norm{\Sigma}$ denotes the operator norm. (the largest eigenvalue since $\Sigma$ is symmetric)
\end{corollary}

\begin{proof}
We start by noting some of the immediate corollaries of the assumption:

\begin{equation*} \label{eq:delbound} \tag{I}
    | \alpha \Delta^\top (\hat{\Sigma}_i - \Sigma) \alpha \Delta | \leq C(\kappa) \alpha^2 \Delta^\top \Sigma \Delta = \alpha^2 C(\kappa) \norm{\Delta}_\Sigma^2
\end{equation*}{}


\begin{equation*} \label{eq:vbound} \tag{II}
  | v^\top (\hat{\Sigma}_i - \Sigma) v |  \leq C(\kappa) v^\top \Sigma v \leq C(\kappa) \norm{\Sigma}  
\end{equation*}{}

\begin{equation*} \label{eq:sumbound} \tag{III}
    |(\alpha \Delta + v)^\top (\hat{\Sigma}_i - \Sigma) (\alpha \Delta + v)| \leq C(\kappa) (\alpha \Delta + v)^\top \Sigma (\alpha \Delta + v) =  C(\kappa) \norm{(\alpha \Delta + v)}_\Sigma^2 \leq 2 C(\kappa) (\alpha^2 \norm{\Delta}_\Sigma^2 + \norm{\Sigma})
\end{equation*}{}

where we note that $\norm{v}_\Sigma^2 = \norm{\Sigma}$ and we have used the fact that $\norm{a +b}^2 \leq 2(\norm{a}^2 + \norm{b}^2)$

Now, let's just look at the upper bound, the lower bound follows analogously; expanding out the last term we get that 

$(\alpha \Delta + v)^\top (\hat{\Sigma}_i - \Sigma) (\alpha \Delta + v) = (\alpha \Delta)^\top  (\hat{\Sigma}_i - \Sigma) \alpha \Delta + 2 (\alpha \Delta)^\top (\hat{\Sigma}_i - \Sigma) v + v^\top (\hat{\Sigma}_i - \Sigma) $

where we have used the symmetry of $(\hat{\Sigma}_i - \Sigma)$ to reduce  $(\alpha \Delta)^\top (\hat{\Sigma}_i - \Sigma) v = v^\top (\hat{\Sigma}_i - \Sigma) \alpha \Delta $ 

By \eqref{eq:sumbound} before, we have that:

\begin{equation*}
(\alpha \Delta)^\top  (\hat{\Sigma}_i - \Sigma) \alpha \Delta + 2 (\alpha \Delta)^\top (\hat{\Sigma}_i - \Sigma) v + v^\top (\hat{\Sigma}_i - \Sigma) \leq 2 C(\kappa) (\alpha^2 \norm{\Delta}_\Sigma^2 + \norm{\Sigma})
\end{equation*}{}

so rearranging, and using \eqref{eq:vbound} and \eqref{eq:delbound}, we get that 

\begin{equation*}
2 (\alpha \Delta)^\top (\hat{\Sigma}_i - \Sigma) v \leq  2 C(\kappa) (\alpha^2 \norm{\Delta}_\Sigma^2 + \norm{\Sigma}) +  C(\kappa) \norm{\Sigma}  +  \alpha^2 C(\kappa) \norm{\Delta}_\Sigma^2
\end{equation*}{}

and after simplifying, we get that 

\begin{equation*}
(\Delta)^\top (\hat{\Sigma}_i - \Sigma) v \leq  \frac{3}{2} C(\kappa) \alpha \norm{\Delta}_\Sigma^2 + \frac{1}{\alpha}\norm{\Sigma})
\end{equation*}{}

Now, optimizing over $\alpha$, we get that the optimal $\alpha = \frac{\sqrt{\norm{\Sigma}}}{\norm{\Delta}_\Sigma}$ allows us to reduce the bound to 

\begin{equation*}
(\Delta)^\top (\hat{\Sigma}_i - \Sigma) v \leq  3 C(\kappa) \norm{\Delta}_\Sigma \sqrt{\norm{\Sigma}}
\end{equation*}{}

\end{proof}

We take first half of the following lemma 2.1 from \cite{mendelson2018robust} in verbatim:

\begin{lemma}
If $X$ is zero mean and satisfies an $L_4-L_2$ norm equivalence with constant $L$, then 
$$\| \tilde { \Sigma } - \Sigma \| \leq c ( L ) \frac { \| \Sigma \| \operatorname { Tr } ( \Sigma ) } { \alpha ^ { 2 } }$$
\end{lemma}{}

Let's introduce some notation; let $A$ be a symmetric positive definite matrix; we will use $\lmin(A)$ and $\lmax(A)$ to denote the minimum and maximum eigenvalues of $A$, and $\kappa(A) := \frac{\lmax(A)}{\lmin(A)}$ to denote the condition number of $A$. 

We note that the following simple lemma allows us to compare the condition numbers of the truncated population covariance ($\kappa(\tilde{\Sigma})$) with the normal population covariance ($\kappa(\Sigma)$):

\begin{lemma}
If $$\| \tilde { \Sigma } - \Sigma \| \leq \frac{1}{2} \lmin (\Sigma)$$, then
$$ \kappa(\tilde{\Sigma}) \leq 2 \kappa(\Sigma)$$
\end{lemma}{}
\begin{proof}
We note that $\lmax(\tilde{\Sigma}) \leq \lmax(\Sigma)$, since $\Sigma = (\Sigma - \tilde{\Sigma}) + \tilde{\Sigma}$

We also note that $\lmin(\tilde(\Sigma)) \geq \lmin{\Sigma} - \norm{\tilde { \Sigma } - \Sigma}$ by triangle inequality, so combining these with $\frac{a}{b - x} \leq 2\frac{a}{b}$ for $x \in [0, \frac{b}{2}], a, b > 0$, gives the result.  

\end{proof}{}
So now, let's do some term matching. Let's assume that at the end of the day we will need the same upper bound constraint on $\alpha$ that they get so that matrix Bernstein works, that is, equation (26) from \cite{minsker2018robust}:

$$\alpha \leq c _ { 2 } ( L ) \left( \frac { \operatorname { Tr } ( \Sigma ) \| \Sigma \| N } { \log \mathbf { r } ( \Sigma ) } \right) ^ { \frac { 1 } { 4 } }$$,

which gives us:

$$c ( L ) \frac { \| \Sigma \| \operatorname { Tr } ( \Sigma ) } { \alpha ^ { 2 } } \geq  \| \Sigma \| \operatorname { Tr } ( \Sigma )  c _ { 2 } ( L ) \left( \frac { \operatorname { Tr } ( \Sigma ) \| \Sigma \| N } { \log \mathbf { r } ( \Sigma ) } \right) ^ { -\frac { 1 } { 2 } }$$.

To play heuristically, let's set all these inequalities to equalities, and then set the trace of $\Sigma$ and the effective rank of $\Sigma$ to be of order $d$.

We then get that the lemma 2.1 gives us 

$$\| \tilde { \Sigma } - \Sigma \| \leq c(L) \sqrt{\frac{\norm{\Sigma} d \log d}{N}} $$,

so to get a nice control over the condition number, we need that 

$$c(L) \sqrt{\frac{\norm{\Sigma} d \log d}{N}} \leq \frac{1}{2} \lmin(\Sigma)$$,
or, rearranging, we get 

$$ N \geq d \log d (\kappa(\Sigma))^2 \norm{\Sigma} $$

\begin{lemma}
    Let $X$ be $n$ iid random vectors satisfying $L_4 - L_2$ norm equivalence with constant $L$, then we have:
    
    \begin{equation*}
        \mathbb{E} [\norm{X}^4] \leq L \cdot (\Tr \Sigma)^2
    \end{equation*}
\end{lemma}

\begin{proof}
    We have:
    \begin{equation*}
        \mb{E} [\norm{X}^4] = \sum_{i,j} \mb{E} [X_i^2 X_j^2] \leq \sum_{i, j} \lprp{\mb{E} [X_i^4] \mb{E} [X_j^4]}^{1 / 2} \leq L \sum_{i, j} \mb{E} [X_i^2] \mb{E} [X_j^2] = L \cdot (\Tr \Sigma)^2
    \end{equation*}
\end{proof}



\begin{proof}
    Let 
\end{proof}
